The OxyContin Reformulation Revisited: New Evidence From Improved Definitions of Markets and Substitutes

The opioid epidemic began with prescription pain relievers. In 2010 Purdue Pharma reformulated OxyContin to make it more difficult to abuse. OxyContin misuse fell dramatically, and concurrently heroin deaths began to rise. Previous research overlooked generic oxycodone and argued that the reformulation induced OxyContin users to switch directly to heroin. Using a novel and fine-grained source of all oxycodone sales from 2006-2014, we show that the reformulation led users to substitute from OxyContin to generic oxycodone, and the reformulation had no overall impact on opioid or heroin mortality. In fact, generic oxycodone, instead of OxyContin, was the driving factor in the transition to heroin. Finally, we show that by omitting generic oxycodone we recover the results of the literature. These findings highlight the important role generic oxycodone played in the opioid epidemic and the limited effectiveness of a partial supply-side intervention.

==> table3_DID.tex <==
\begin{center}
\caption{Difference in difference regression results}
\label{tab:did}
\begin{tabular} {L{0.3\textwidth}C{0.13\textwidth}C{0.13\textwidth}C{0.13\textwidth}C{0.13\textwidth}}
\hline\hline
 & \multicolumn{2}{c}{Opioid sales per person} & \multicolumn{2}{c}{Overdose per 10,000} \\ \cline{2-5}
 & OxyContin & Oxycodone & Opioid & Heroin \\
 & (1) & (2) & (3) & (4) \\ \hline
Post & -8.05 & 41.74 & 0.01 & 0.14 \\
 & (2.18) & (5.43) & (0.02) & (0.01) \\
High OxyContin & 47.24 & 56.46 & -0.05 & -0.07 \\
 & (2.24) & (5.58) & (0.02) & (0.01) \\
High Oxycodone & 26.84 & 95.90 & 0.14 & 0.08 \\
 & (2.79) & (6.95) & (0.02) & (0.02) \\
Post x High OxyContin & -15.14 & 10.30 & 0.02 & 0.03 \\
 & (2.46) & (6.13) & (0.02) & (0.02) \\
Post x High Oxycodone & -2.33 & 33.99 & 0.06 & 0.07 \\
 & (2.45) & (6.11) & (0.02) & (0.02) \\
Number of observations & 2148 & 2148 & 2148 & 2148 \\
R-square & 0.665 &  0.737 & 0.517 & 0.469 \\
Adjusted R-square & 0.654 & 0.728 & 0.501 & 0.452 \\\hline
\end{tabular}

\begin{tablenotes}
      \small
      \item \textit{Notes:} We report coefficients from the difference-in-difference estimation (see equation (3)). All MSAs in Florida are excluded. In all specifications, we include MSA-level control variables, state fixed effects and year fixed effects.
\end{tablenotes}

\end{center}
